PrivateGaze: Preserving User Privacy in Black-box Mobile Gaze Tracking Services

Eye gaze contains rich information about human attention and cognitive processes. This capability makes the underlying technology, known as gaze tracking, a critical enabler for many ubiquitous applications and has triggered the development of easy-to-use gaze estimation services. Indeed, by utilizing the ubiquitous cameras on tablets and smartphones, users can readily access many gaze estimation services. In using these services, users must provide their full-face images to the gaze estimator, which is often a black box. This poses significant privacy threats to the users, especially when a malicious service provider gathers a large collection of face images to classify sensitive user attributes. In this work, we present PrivateGaze, the first approach that can effectively preserve users' privacy in black-box gaze tracking services without compromising gaze estimation performance. Specifically, we proposed a novel framework to train a privacy preserver that converts full-face images into obfuscated counterparts, which are effective for gaze estimation while containing no privacy information. Evaluation on four datasets shows that the obfuscated image can protect users' private information, such as identity and gender, against unauthorized attribute classification. Meanwhile, when used directly by the black-box gaze estimator as inputs, the obfuscated images lead to comparable tracking performance to the conventional, unprotected full-face images.

==> Backups/05method_backup_v1.tex <==
% \section{Problem Formulation}
% \subsection{Black-box Gaze Estimation Services}
% We consider to preserve user privacy when calling the black-box gaze estimation services. In detail, the untrusted third party provides the gaze estimation services to users by receiving facial images from users and returning the estimated gaze directions. The gaze estimation services are achieved by a deep learning-based gaze estimator, which is a black box to users and trained by the untrusted third party on an unknown dataset $\mathcal{D}_{b}$.  We use $\mathcal{G}_b(\cdot)$ to denote the black-box gaze estimator.

% \subsection{Assumptions}
% We assume to be able to access to a public available gaze dataset $\mathcal{D}_{w}$ that contains training examples $(x_i,g_i)$, where $x_i$ is the facial image and $g_i$ is the gaze annotation. Note that, $\mathcal{D}_{w}$ is different with $\mathcal{D}_{b}$ as we do not know which dataset is used by the third party to train $\mathcal{G}_b(\cdot)$. We also assume that we do not need to consider the privacy attributes contained in the $\mathcal{D}_{w}$, as $\mathcal{D}_{w}$ is public available.

% \subsection{Our Goals}

% We aim to design an privacy preserver $\mathcal{P}(\cdot)$ to preserve the privacy contained in the raw image collcted from users in black-box gaze estimation services. $\mathcal{P}(\cdot)$ takes inputs raw images from users and outputs converted images, which have the same size of the raw images and satisfy the requirement of input size of $\mathcal{G}_b(\cdot)$. The users call the gaze estimation services with the converted images instead of the raw images. There are two goals for preserving user privacy. First, we hope the converted images do not contain privacy attributes, such as identities. We term the first goal as \emph{privacy purpose}. Second, we hope the gaze estimation performance of $\mathcal{G}_b(\cdot)$ on converted images is similar with that on raw images. We term the second goal as \emph{utility purpose}. 

% To achieve the privacy purpose and utility purpose, we propose {\name}. The key

\section{Method}
\textcolor{blue}{In this section, we introduce {\name} to preserve user privacy in black-box gaze estimation services. We first formulate the problem. We then give a detailed design of {\name}.}

\subsection{Problem Formulation}

% We aim to preserve the user's privacy in the following practical scenario. 

We consider the scenario where a user would like to use the gaze estimation service provided by a third party. The service provider takes the full-face images of the user as the input and returns with the estimated gaze directions. Unlike existing works~\cite{wu2021dapter, 8658803, 10.1145/3369816, DeepObfuscator} that assume the details of the deep neural network used by the service provider are known, we consider a more practical case where the gaze estimation is performed by a black-box, deep learning-based model that is trained on an unknown dataset: the user can only query and request the black-box gaze estimator for service and has no knowledge about its implementation and training details. We use $\mathcal{G}_b(\cdot)$ to denote the %well-trained gaze estimator and call it the 
\emph{black-box gaze estimator} and denote the unknown training dataset as $\mathcal{D}_{b}$. Note that, the end-to-end estimation system, i.e., the processing pipeline and the deep learning-based estimation model, can be running on either a local device of the user or remotely on a cloud server owned by the service provider. Such an opaque design makes the gaze estimation service untrustworthy, as the full-face image of the user can be illegally used for other purposes that are beyond gaze estimation, i.e., inferring the user's private attributes such as identity and gender. Thus, the user would like to remove the private information contained in the full-face images before sharing them with the service provider, without sacrificing gaze estimation performance.


% We consider preserving user privacy in the following scenario. The untrusted third party provides black-box gaze estimation service by receiving facial images from users and returning the estimated gaze directions. The black-box gaze estimation services infer gaze directions from the received facial image by a well-trained gaze estimator that is trained by the untrusted third party on an unknown dataset $\mathcal{D}_{b}$. We use $\mathcal{G}_b(\cdot)$ to denote the well-trained gaze estimator and call it the \emph{black-box gaze estimator}. Note that the users can only query the black-box gaze estimator and do not know the details about the black-box gaze estimator, such as structures and parameters. As the users do not know whether the black-box gaze estimation services use the received facial image for other purposes beyond gaze estimation, such as inferring the private attributes of users, the users expect to remove the private attributes, e.g., identities and gender, contained in the raw images before calling the black-box gaze estimation services. Meanwhile, the users expect to receive accurate gaze directions from $\mathcal{G}_b(\cdot)$ by using images without private information.

%To preserve private attributes contained in raw images, the users call the black-box gaze estimation services by sending converted images instead of raw images. The converted images are transformed from raw images and should possess the following two properties. First, the converted images do not contain private attributes of users, such as identities. We term this property as \emph{privacy} Second, the converted images can be directly by $\mathcal{G}_b(\cdot)$ and the gaze estimation performance of $\mathcal{G}_b(\cdot)$ on converted images should be similar with that on raw images. 

\textbf{Design goals.} In this work, we play the role of a more trustworthy party and provide a transparent privacy preserver $\mathcal{P}(\cdot)$ that can be deployed on the user's device. As shown in Figure~\ref{Fig:teaser_figure}, in the deployment stage, the privacy preserver takes the original full-face images of the user and converts them into anonymized images that do not contain any user attributes, e.g., identity and gender. The converted images are then used as inputs for the black-box gaze estimation. Formally, the converted images must fulfill the objectives of preserving the user's privacy while ensuring good gaze estimation performance: 
\begin{itemize}
\setlength\itemsep{0.6em}
    \item \textbf{Privacy goal:} the converted images cannot be used by the third-party service provider to infer private attributes of the user, such as identity and gender.
    \item \textbf{Utility goal:} the converted images can be directly used by the black-box gaze estimator $\mathcal{G}_b(\cdot)$ without any adaption needed from the service provider's side; and the gaze estimation performance of $\mathcal{G}_b(\cdot)$ on the converted images should be similar with that on the raw images.
\end{itemize}

% In this work, we play a role as a trusted party, which aims to design a privacy preserver $\mathcal{P}(\cdot)$ that will be deployed on the user side. The privacy preserver transforms raw images from users into converted images, and the users call the black-box gaze estimation services with the converted images instead of the raw images. Formally, the converted images should possess the following two objectives to preserve user privacy: \begin{itemize}
%     \item \textbf{Privacy:} The converted images do not contain private attributes of users, such as identities and genders.
%     \item \textbf{Utility:} The converted images can be directly used by $\mathcal{G}_b(\cdot)$ and the gaze estimation performance of $\mathcal{G}_b(\cdot)$ on converted images should be similar with that on raw images.
% \end{itemize}

\textbf{Assumption.} We assume we have access to a publicly available gaze estimation dataset $\mathcal{D}_{w}$ that contains training examples $(x_i,g_i)$, where $x_i$ is the full-face image and $g_i$ is the corresponding gaze annotation. Note that $\mathcal{D}_{w}$ is different from $\mathcal{D}_{b}$ as we do not know which dataset has been used by the service provider to train the black-box gaze estimator. %$\mathcal{G}_b(\cdot)$. 
The dataset $\mathcal{D}_{w}$ will be used to train the privacy preserver $\mathcal{P}(\cdot)$. 

% \textbf{Assumption.} To obtain a privacy preserver $\mathcal{P}(\cdot)$ to achieve privacy objective and utility objective, we assume to be able to access a publicly available gaze dataset $\mathcal{D}_{w}$ that contains training examples $(x_i,g_i)$, where $x_i$ is the facial image and $g_i$ is the gaze annotation. Note that $\mathcal{D}_{w}$ is different from $\mathcal{D}_{b}$ as we do not know which dataset is used by the third party to train $\mathcal{G}_b(\cdot)$.




\subsection{Design Overview of {\name}}

% In this work, we propose {\name}, which trains a privacy preserver that can achieve both privacy and utility goals. Specifically, to fulfill the privacy requirement, {\name} ensures that the images converted by the privacy preserver share a similar appearance with a pre-generated \emph{anchor image}. 

% We propose {\name} to train a privacy preserver to achieve both privacy objective and utility objective when users call the black-box gaze estimation services. The privacy preserver takes raw images from users as inputs to generate converted images. To achieve the privacy objective, {\name} requires the converted images to have similar appearances to a pre-generated \emph{anchor image}, which is an average facial image generated from $\mathcal{D}_{w}$. In this way, the converted images transformed from different raw images have similar appearances. Thus, the private attributes contained in raw images are reserved for users. Since the black-box gaze estimator $\mathcal{G}_b(\cdot)$ cannot be included in the training loop for backpropagation, {\name} trains a surrogate gaze estimator $\mathcal{G}_w(\cdot)$ on $\mathcal{D}_{w}$ to replace $\mathcal{G}_b(\cdot)$ in the training stage. 

We propose {\name} to achieve both privacy and utility goals. First, to fulfill the privacy requirement, we aim to ensure that all the converted images, once transformed from the original full-face images, have the same facial appearance. A naive solution is to maximize the similarity between each converted image pair. However, it will make the final appearance of the converted images unpredictable and lead to poor performance on the black-box gaze estimation model. Second, to achieve the utility objective, we need to ensure that the converted images contain the essential image features to enable good gaze estimation performance. %, such that they can achieve good accuracy when used for gaze estimation. 
However, %{unlike existing works~\cite{wu2021dapter, 8658803, 10.1145/3369816, DeepObfuscator} that assume the details of the deep neural network used by the service provider are known, we consider a more practical scenario where 
as the gaze estimator $\mathcal{G}_b(\cdot)$ is a black-box model, it is impossible to include it in the training loop of the privacy preserver and assist in identifying the necessary features. 

To resolve these challenges, {\name} first trains a surrogate gaze estimator $\mathcal{G}_w(\cdot)$ on the publicly available gaze estimation dataset $\mathcal{D}_{w}$ to replace $\mathcal{G}_b(\cdot)$ in the training stage. Moreover, {\name} devises a method for generating an anchor image that synthesizes an average face by blending images selected from $\mathcal{D}_{w}$. Specifically, the images are selected by querying both $\mathcal{G}_w(\cdot)$ and $\mathcal{G}_b(\cdot)$, and ensure both models exhibit the same gaze estimation behavior on the final anchor image. The anchor image is then utilized to guide the training of the privacy preserver, enabling it to transform all original, privacy-sensitive images to match the appearance of the anchor image while retaining distinct image features pertinent to gaze direction. Note that, as the dataset $\mathcal{D}_{w}$ used in generating the anchor image does not contain any images of the actual users, this allows us to protect the private attributes of the user. Moreover, as the converted images have a similar appearance to the anchor image, i.e., a minimum gap between their feature distributions, we can ensure they can achieve similar gaze estimation performance on both surrogate and black-box models. This, in turn, ensures that the privacy preserver, which was trained with the surrogate model, produces converted images that maintain good utility when applied to the black-box model.


% Moreover, as the converted images are similar to the anchor image, we can ensure they achieve similar gaze estimation performance on both surrogate and black-box models. This, in turn, ensures that the privacy preserver, which was trained with the surrogate model, produces converted images that maintain good utility when applied to the black-box model.


% \textcolor{blue}{To achieve the utility objective, we must ensure that the converted images contain the gaze features that are essential for gaze estimation, such that when taken as the inputs for gaze estimation, the surrogate gaze estimator can still obtain accurate gaze directions. Moreover, by carefully generating the anchor image $\hat{x}$, {\name} ensures the converted images also make the black-box gaze estimator return accurate gaze directions.}
 
 
% {There are various ways of generating the anchor image, e.g., XXX and XXX,} in this work, we leverage an average face image blended from the publicly available gaze estimation dataset $\mathcal{D}_{w}$ as the anchor image. Note that, $\mathcal{D}_{w}$ does not contain any images of the actual users. Thus, {\name} reserves the users' private attributes by ensuring that all user's images, once converted from the original full-face images, have nearly the same appearance. {Unlike existing works~\cite{wu2021dapter, 8658803, 10.1145/3369816, DeepObfuscator} that assume the details of the deep neural network are known, we consider a more practical scenario where the gaze estimator $\mathcal{G}_b(\cdot)$ is a black-box. Thus, it is impossible to include $\mathcal{G}_b(\cdot)$ in the training loop for back-propagation.} 

% To resolve this problem, {\name} trains a surrogate gaze estimator $\mathcal{G}_w(\cdot)$ on $\mathcal{D}_{w}$ to replace $\mathcal{G}_b(\cdot)$ in the training stage. \textcolor{blue}{To achieve the utility objective, {\name} ensures that the converted images contain the gaze features that are essential for gaze estimation, such that when taken as the inputs for gaze estimation, the surrogate gaze estimator can still obtain accurate gaze directions. Moreover, by carefully generating the anchor image $\hat{x}$, {\name} ensures the converted images also make the black-box gaze estimator return accurate gaze directions.}

% We propose {\name} to train a privacy preserver to achieve both privacy objective and utility objective when users call the black-box gaze estimation services. The privacy preserver takes raw images from users as inputs to generate converted images. To achieve the privacy objective, {\name} requires the converted images to have similar appearances to a pre-generated \emph{anchor image}, which is an average facial image generated from $\mathcal{D}_{w}$. In this way, the converted images transformed from different raw images have similar appearances. Thus, the private attributes contained in raw images are reserved for users. Since the black-box gaze estimator $\mathcal{G}_b(\cdot)$ cannot be included in the training loop for backpropagation, {\name} trains a surrogate gaze estimator $\mathcal{G}_w(\cdot)$ on $\mathcal{D}_{w}$ to replace $\mathcal{G}_b(\cdot)$ in the training stage. 

% Then, to achieve the utility objective, {\name} maintains the gaze features of raw images for the converted images, such that the converted images make the surrogate gaze estimator return accurate gaze directions. Moreover, by carefully generating the anchor image $\hat{x}$, {\name} ensures the converted images also make the black-box gaze estimator return accurate gaze directions.

Figure \ref{Fig:Overview} shows an overview of {\name}. The privacy preserver $\mathcal{P}(\cdot)$ includes the gaze-feature extractor $F(\cdot)$, the pre-generated anchor image $\hat{x}$, and the image generator $IG(\cdot)$. First, the gaze-feature extractor $F(\cdot)$ extracts gaze features $z_i$ from the original full-face image $x_i$. Next, the image generator $IG(\cdot)$ takes the extracted gaze features $z_i$ and the anchor image $\hat{x}$ as inputs to generate the converted image $x'_i$. Then, the converted image $x'_i$ is sent to the surrogate gaze estimator to obtain the estimated gaze directions $g'_i$. {\name} trains $F(\cdot)$ and $IG(\cdot)$ jointly on $\mathcal{D}_{w}$ to achieve both the privacy and utility objectives. 
Specifically, {\name} introduces the \emph{privacy loss} to maximize the similarity between the converted image $x'_i$ and the anchor image $\hat{x}$ to preserve user privacy. Moreover, {\name} devises the \emph{utility loss} to encourage the privacy preserver to generate $x'_i$ that can make the estimated gaze $g'_i$ close to the ground truth $g_i$. \textcolor{blue}{In the rest of this section, we introduce XXX}

\begin{figure}[]
  \centering
  \includegraphics[width=0.99\linewidth]{Figures/Overview.pdf}
  \caption{Overview of {\name}. The %raw image is fed into the 
  privacy preserver includes the gaze-feature extractor, the image generator, and the anchor image $\hat{x}$. First, the gaze-feature extractor extracts gaze features $z_i$ from the raw image $x_i$. Then, the image generator takes the anchor image $\hat{x}$ and $z_i$ as inputs to generate the converted image $x'_i$. After that, we calculate the \textit{privacy loss} based on $\hat{x}$ and $x'_i$ to train the privacy preserver for the privacy objective. %Since the black-box gaze estimator cannot be included in the training loop, 
  We train a surrogate gaze estimator to replace the black-box gaze estimator in the training stage. Next, $x'_i$ is sent to the surrogate gaze estimator to obtain the estimated gaze direction $g'_i$. Finally, we calculate the \textit{utility loss} based on the gaze annotation $g_i$ and $g'_i$ to train the privacy preserver for the utility objective.}
  \label{Fig:Overview}
  \vspace{-0.1in}
\end{figure}

\subsection{Structure of Privacy Preserver}

Below, we introduce the design of the privacy preserver. As shown in Figure~\ref{Fig:PrivacyPreserver}, it consists of the gaze-feature extractor, %the generation of 
the anchor image, and the image generator. 

% \subsubsection{Gaze-feature extractor.} The purpose of the gaze-feature extractor $F(\cdot)$ is to extract gaze features $z_i$ from the raw image $x_i$. As is shown in the left part of Figure~\ref{Fig:PrivacyPreserver}, the gaze-feature extractor consists of the gaze-aware encoder $E(\cdot)$ and the gaze projector $G(\cdot)$. In detail, $E(\cdot)$ takes the raw image $x_i$ as input and outputs a feature vector $z_i$. Then, to encourage $E(\cdot)$ to extract gaze features, $z_i$ is fed into a nonlinear gaze projector $G(\cdot)$ to obtain the estimated gaze direction, where $G(\cdot)$ is implemented by a pooling layer followed by a flatten layer and two fully connected layers. We define the following gaze estimation loss to train $E(\cdot)$ and $G(\cdot)$:
% \begin{equation}
%     \mathcal{L}_g=\sum_{(x_i,g_i)\in\mathcal{D}_w}\ell(G(E(x_i)),g_i),
%     \label{Eq:gaze_mlp}
% \end{equation}where $\ell(\cdot)$ is $L_1$ loss function. Note that, only the gaze features $z_i$ are sent to the image generator, and the gaze projector $G(\cdot)$ will be discarded in the inference stage.

\subsubsection{Gaze-feature extractor.} The purpose of the gaze-feature extractor $F(\cdot)$ is to extract gaze features $z_i$ from the raw image $x_i$. As shown in the left part of Figure~\ref{Fig:PrivacyPreserver}, the gaze-feature extractor consists of the gaze-aware encoder $E(\cdot)$ and the gaze projector $G(\cdot)$. In detail, $E(\cdot)$ takes the raw image $x_i$ as input and outputs a feature vector $z_i$. Then, to encourage $E(\cdot)$ to extract gaze features, $z_i$ is fed into a nonlinear gaze projector $G(\cdot)$ to obtain the estimated gaze direction, where $G(\cdot)$ is implemented by a pooling layer followed by a flatten layer and two fully connected layers. We define the following gaze estimation loss to train $E(\cdot)$ and $G(\cdot)$:
\begin{equation}%\large
    \mathcal{L}_g=\sum_{(x_i,g_i)\in\mathcal{D}_w}\ell(G(E(x_i)),g_i),
    \label{Eq:gaze_mlp}
\end{equation}
where $\ell(\cdot)$ is $L_1$ loss function. Note that, only the gaze features $z_i$ are sent to the image generator, and the gaze projector $G(\cdot)$ will be discarded in the inference stage.

\subsubsection{Image generator.} Image generator $IG(\cdot)$ aims to generate the converted image $x'_i$ that has a similar appearance to the anchor image but maintains the gaze features of the raw image $x_i$. To achieve this goal, we design $IG(\cdot)$ to take both $z_i$ and $\hat{x}$ as inputs to generate the converted image $x'_i$.
The structure of $IG(\cdot)$ is illustrated in the right part of Fig. \ref{Fig:PrivacyPreserver}, which includes an encoder and a decoder. First, the encoder takes the anchor image $\hat{x}$ as input and outputs the features $\hat{z}$, which have the same spatial size as $z_i$. The encoder includes several convolutional blocks (Conv Block). Then, $IG(\cdot)$ concatenates the gaze features $z_i$ extracted from $x_i$ with $\hat{z}$, and feeds the concatenated features to the decoder to generate the converted image $x'_i$. The decoder consists of several up-convolutional blocks (Up-conv Block) and each Up-conv Block consists of the upsampling of the feature map followed by several convolutional layers. In order to encourage the decoder to generate an image that is similar to the anchor image, $IG(\cdot)$ concatenates the output of each Up-conv Block with the corresponding feature map in the encoder and feeds the concatenated feature map to the next Up-conv Block, as is shown in Fig. \ref{Fig:PrivacyPreserver}. We use $x'_i=IG(\{z_i,\hat{x}\})$ to denote the process of generating the converted image $x'_i$ from $z_i$ and $\hat{x}$. Note that, despite using three Conv Blocks and three Up-conv Blocks to illustrate the structure of $IG(\cdot)$, in practice, we can vary the number of Conv Blocks and Up-conv Blocks.

\begin{figure}[]
  \centering
  \includegraphics[width=0.53\linewidth]{Figures/PrivacyPreserver.pdf}
  \caption{The structure of privacy preserver. The privacy preserver consists of the gaze-feature extractor, the anchor image, and the image generator. The gaze-feature extractor extracts gaze features $z_i$ from the raw image $x_i$ of the user. The image generator takes the extracted gaze features $z_i$ and the anchor image $\hat{x}$ as inputs to generate the converted image. The converted image has a similar appearance to the anchor image but maintains the gaze features of the raw image.}
  \label{Fig:PrivacyPreserver}
  \vspace{-0.1in}
\end{figure}

\subsubsection{Generation of anchor image}
We carefully generate the anchor image to ensure the privacy preserver trained with the surrogate gaze estimator $\mathcal{G}_w(\cdot)$ can be generalized to the black-box gaze estimator $\mathcal{G}_b(\cdot)$. That is, the converted image generated by the privacy preserver can make both the surrogate gaze estimator and the black-box gaze estimator return accurate gaze directions. First, as the black-box gaze estimator and the surrogate gaze estimator are trained on facial images, we generate a facial image as the anchor image. Second, we use an average facial image generated from several facial images in the training dataset as the anchor image, since we hope the converted images do not look like a specific subject. Lastly, we generate an anchor image that can lead to similar outputs of $\mathcal{G}_w(\cdot)$ and $\mathcal{G}_b(\cdot)$.

In detail, we first randomly sample $N$ raw images $\{x_i\}_{i=1}^N$ from the training dataset and query $\mathcal{G}_w(\cdot)$ and $\mathcal{G}_b(\cdot)$ with $\{x_i\}_{i=1}^N$ to obtain the estimated gaze directions $\{\mathcal{G}_w(x_i)\}_{i=1}^N$ and $\{\mathcal{G}_b(x_i)\}_{i=1}^N$ respectively. Then, we calculate the $L1$ norm between the gaze directions estimated by $\mathcal{G}_w(\cdot)$ and $\mathcal{G}_b(\cdot)$ for each image $x_i$ to obtain the list $\{D_g(x_i)\}_{i=1}^N$, where $D_g(x_i)=|\mathcal{G}_w(x_i)-\mathcal{G}_b(x_i)|_1$. After that, we sort the list $\{D_g(x_i)\}_{i=1}^N$ in the ascending order. We use $\{x_k\}_{k=1}^N$ to denote the set of raw images after sorting, which satisfies $D_g(x_k)\leq D_g(x_{k+1})$. We use $Ave(m)$ to denote the average facial image calculated from the first $m$ images in $\{x_k\}_{k=1}^N$ by $Ave(m)=\frac{1}{m}\sum_{k=1}^{m}x_k$. We generate $M$ average facial images by varying $m$ from $K_1$ to $K_1+M$, where $K_1>1$ and $K_1+M\leq N$. Finally, we query $\mathcal{G}_w(\cdot)$ and $\mathcal{G}_b(\cdot)$ with the $M$ average facial images and select the one that leads to the minimum $L_1$ norm between the outputs of $\mathcal{G}_w(\cdot)$ and $\mathcal{G}_b(\cdot)$ as the anchor image. We set $K_1=15$, $M=35$, and $N=500$. %, as we hope the anchor image do not look like a specific subject. We set $M=35$ and $N=500$.
The anchor image obtained from GazeCapture dataset \cite{Krafka_2016_CVPR} is shown in Fig. \ref{Fig:PrivacyPreserver}. %$We perform ablation study to investigate the impact of $M$ and $N$ on the performance of {\name} in the evaluation section.


\subsection{Training of Privacy Preserver}
Below, we introduce the loss function used to train the privacy preserver to achieve the privacy objective and the utility objective.
\subsubsection{Privacy Loss.} To achieve the privacy objective, {\name} requires the converted images to be similar to the anchor image $\hat{x}$. Consequently, the converted images transformed from different raw images will have similar appearances, i.e., the appearance of the anchor image. Thus, the private attributes contained in the raw images are reserved for the users. Formally, in order to achieve the privacy objective, {\name} introduces the following loss function to maximize the similarity between the converted images and the anchor image: \begin{equation}
    \mathcal{L}_{privacy} = \sum_{(x_i,g_i)\in\mathcal{D}_{w}}1-\text{MS-SSIM}\left(\hat{x},IG\left(\{E(x_i),\hat{x}\}\right)\right),
\end{equation}where $\text{MS-SSIM}(\cdot,\cdot)$ \cite{1292216} is a function to measure the similarity between two images and its value is in the range of $[0,1]$. The larger value of $\text{MS-SSIM}$ indicates a higher similarity between the two images. {\name} terms $\mathcal{L}_{privacy}$ as the privacy loss. 

\subsubsection{Utility loss.} To achieve the utility objective, {\name} feeds the converted image $x'_i$ to the surrogate gaze estimator $\mathcal{G}_{w}(\cdot)$ to obtain the estimated gaze direction $g'_i$ for $x'_i$ and trains the privacy preserver to make $g'_i$ close to $g_i$.
%{\name} expects the black-box gaze estimator $\mathcal{G}_{b}(\cdot)$ to output the gaze direction $g_i$ when taking $x'_i$ as input. However, since $\mathcal{G}_{b}(\cdot)$ cannot be used for backpropagation in the training stage, {\name} trains a surrogate gaze estimator $\mathcal{G}_{w}(\cdot)$ on $\mathcal{D}_{w}$ and trains the privacy preserver to make $\mathcal{G}_{w}(\cdot)$ output $g_i$ for $x'_i$. 
Besides, the gaze estimation loss $\mathcal{L}_g$ defined in Equation \ref{Eq:gaze_mlp} can encourage the extraction of gaze features from the raw images, which also contributes to the utility objective. Formally, {\name} defines the following utility loss to train the privacy preserver for utility objective:
\begin{equation}
    \mathcal{L}_{utility}=\sum_{(x_i,g_i)\in\mathcal{D}_{w}}\ell\left(\mathcal{G}_{w}\left(IG\left(\{E(x_i),\hat{x}\}\right)\right),g_i\right) + \mathcal{L}_g,
    \label{Eq:utility_white}
\end{equation}where $\ell(\cdot)$ is $L_1$ loss function. The first term of $\mathcal{L}_{utility}$ aims to minimize the $L_1$ norm between $\mathcal{G}_{w}(x'_i)$ and $g_i$, while the second term encourages to extract gaze features for generating the converted image $x'_i$.


\subsubsection{Optimization objective} The final optimization objective is the weighted sum of $\mathcal{L}_{utility}$ and $\mathcal{L}_{privacy}$:
\begin{equation}
\mathcal{L} = \mathcal{L}_{utility} + \lambda\mathcal{L}_{privacy},
\label{Eq:loss_function}
\end{equation}where $\lambda$ is the weight for the purpose of a trade-off between utility objective and privacy objective. {\name} trains the parameters of $F(\cdot)$ and $IG(\cdot)$ by minimizing $\mathcal{L}$. By default, {\name} set $\lambda=75$. We perform ablation studies to investigate the impact of $\lambda$ on the performance of {\name} in the evaluation section.

\subsection{Deployment of Privacy Preserver}
In the deployment stage, the raw images collected from users are first transformed into converted images by the trained privacy preserver. The users then call the black-box gaze estimation services with the converted images to preserve privacy. Instead of deploying all the components of the privacy preserver, we only need to deploy several components (colored yellow in Fig. \ref{Fig:PrivacyPreserver}) to the user side to reduce the requirement for computational resources. For the gaze-feature extractor, we only need to deploy the gaze-aware encoder, as the image generator only needs the outputs of the gaze-aware encoder, i.e., gaze features. For the image generator, since the anchor image is fixed for different raw images, we can discard the encoder and store the feature maps generated by each convolutional block of the encoder as the \emph{appearance features}. Then, we only need to deploy the decoder of the image generator and the appearance features to obtain the converted images. We perform system profiling in the evaluation section to show that the privacy preserver can be deployed on various hardware platforms without introducing too much latency.
